A General Method for Robust Learning from Batches

In many applications, data is collected in batches, some of which are corrupt or even adversarial. Recent work derived optimal robust algorithms for estimating discrete distributions in this setting. We consider a general framework of robust learning from batches, and determine the limits of both classification and distribution estimation over arbitrary, including continuous, domains. Building on these results, we derive the first robust agnostic computationally-efficient learning algorithms for piecewise-interval classification, and for piecewise-polynomial, monotone, log-concave, and gaussian-mixture distribution estimation.

==> comments.tex <==
\begin{comment}


\begin{align*}
&\sum_{i\in  U_G}\Big(\frac{\subsetcountbatch}{\bsize}-  q  \Big)^2 = \sum_{i\in  U_G}\Big(\frac{\subsetcountbatch}{\bsize}- \subsetprobbatch +\subsetprobbatch-  q  \Big)^2\\
&= \sum_{i\in  U_G}\Big( \Big(\frac{\subsetcountbatch}{\bsize}- \subsetprobbatch\Big)^2 + 2   \Big(\frac{\subsetcountbatch}{\bsize}- \subsetprobbatch\Big)\Big(\subsetprobbatch-\subsetprobtarget+\subsetprobtarget- q  \Big)+\Big(\subsetprobbatch-  q  \Big)^2\Big)\\
&\le \sum_{i\in  U_G}\Big( \Big(\frac{\subsetcountbatch}{\bsize}- \subsetprobbatch\Big)^2 + \eta \Big|\frac{\subsetcountbatch}{\bsize}- \subsetprobbatch\Big|+2  \Big(\frac{\subsetcountbatch}{\bsize}- \subsetprobbatch\Big)\Big(\subsetprobtarget-  q  \Big)+\Big(\subsetprobbatch-  q  \Big)^2\Big)\\
&\le \sum_{i\in  U_G}\Big( \Big(\frac{\subsetcountbatch}{\bsize}- \subsetprobbatch\Big)^2 +2  \Big(\frac{\subsetcountbatch}{\bsize}- \subsetprobbatch\Big)\Big(\subsetprobtarget-  q  \Big)+\Big(\subsetprobbatch-  q  \Big)^2\Big)\\
&+ \eta \sqrt{ |U_G| \sum_{i\in  U_G} \Big(\frac{\subsetcountbatch}{\bsize}- \subsetprobbatch\Big)^2}\\
&\le  \sum_{i\in  U_G}\Big( \Big(\frac{\subsetcountbatch}{\bsize}- \subsetprobbatch\Big)^2+\Big(\subsetprobbatch-  q  \Big)^2\Big)+ 2 \sqrt{ \sum_{i\in  U_G}\Big(\frac{\subsetcountbatch}{\bsize}- \subsetprobbatch\Big)^2
\sum_{i\in  U_G}\Big(\subsetprobbatch-  q  \Big)^2}\\
& \le |U_G| \Big( \frac{\subsetprobtarget(1-\subsetprobtarget)}{\bsize}+ 24{\frac{ \epsilon\ln (e/\epsilon) } {\bsize}} + \frac{\eta}{2n} + \max_{i\in  U_G} (\subsetprobbatch-  q )^2\Big) \Big)  \\
& +2 |U_G| \sqrt{ \Big( \frac{\subsetprobtarget(1-\subsetprobtarget)}{\bsize} + 24{\frac{ \epsilon\ln (e/\epsilon)} {\bsize}}+\frac \eta {2n} \Big)
\max_{i\in  U_G}\Big(\subsetprobbatch-  q  \Big)^2}\\
&\le |U_G| \Big( \frac{\subsetprobtarget(1-\subsetprobtarget)}{\bsize} + {\frac{24 \epsilon } {\bsize}}\ln \big(\frac e \epsilon\big)+\frac{\eta}{2n} +\max_{i\in  U_G} (\subsetprobbatch-  q )^2 + 2 \sqrt{ \frac{16}{\bsize}}\,
\max_{i\in  U_G}\Big|\subsetprobbatch-  q  \Big|\Big)\\
&\le |U_G| \Big( \frac{\subsetprobtarget(1-\subsetprobtarget)}{\bsize} +{\frac{24 \epsilon } {\bsize}}\ln \big(\frac e \epsilon\big)+\frac{\eta}{2n} +\big(|\subsetprobtarget -  q |+\frac \eta {2}\big)^2 +\frac{8}{\sqrt{ \bsize}}\,
\big(|\subsetprobtarget -  q |+\frac \eta {2}\big) \Big)
\end{align*}

\begin{align*}
&\sum_{i\in  U}\Big(\Big(\frac{\subsetcountbatch}{\bsize}-  q  \Big)^2 -   \frac{q(1-q)}{\bsize} \Big)\\
&\ge |U| \Big( -\frac{|\subsetprobtarget -  q |}{\bsize} - {\frac{24 \epsilon } {\bsize}}\ln \big(\frac e \epsilon\big)-\frac{\eta}{2n} +\big(|\subsetprobtarget -  q |-\frac \eta {2}\big)^2 -\frac{8}{\sqrt{ \bsize}}\,
\big(|\subsetprobtarget -  q |+\frac \eta {2}\big) \Big)
\end{align*}
and 
\begin{align*}
&\sum_{i\in  U}\Big(\Big(\frac{\subsetcountbatch}{\bsize}-  q  \Big)^2 -  \frac{q(1-q)}{\bsize} \Big)\\
&\le |U| \Big( \frac{|\subsetprobtarget -  q |}{\bsize} + {\frac{24 \epsilon } {\bsize}}\ln \big(\frac e \epsilon\big)+\frac{\eta}{2n} +\big(|\subsetprobtarget -  q |+\frac \eta {2}\big)^2 +\frac{8}{\sqrt{ \bsize}}\,
\big(|\subsetprobtarget -  q |+\frac \eta {2}\big) \Big).
\end{align*}
\begin{align*}
&\Bigg|\sum_{i\in  U}\Big(\Big(\frac{\subsetcountbatch}{\bsize}-  q  \Big)^2 -   \frac{q(1-q)}{\bsize} \Big)\Bigg|\\
&\le |U| \Big( \frac{|\subsetprobtarget -  q |}{\bsize} +{\frac{24 \epsilon } {\bsize}}\ln \big(\frac e \epsilon\big)+\frac{\eta}{2n} +\big(|\subsetprobtarget -  q |+\frac \eta {2}\big)^2 +\frac{8}{\sqrt{ \bsize}}\,
\big(|\subsetprobtarget -  q |+\frac \eta {2}\big) \Big).
\end{align*}

\begin{proof}

\begin{align*}
&\sum_{i\in  U}\Big(\frac{\subsetcountbatch}{\bsize}-  q  \Big)^2 = \sum_{i\in  U}\Big(\frac{\subsetcountbatch}{\bsize}- \subsetprobbatch +\subsetprobbatch-  q  \Big)^2\\
&\ge \sum_{i\in  U}\Big( \Big(\frac{\subsetcountbatch}{\bsize}- \subsetprobbatch\Big)^2- 2   \Big|\frac{\subsetcountbatch}{\bsize}- \subsetprobbatch\Big|\Big|\subsetprobbatch-  q  \Big|+\Big(\subsetprobbatch-  q  \Big)^2\Big)\\
&\ge  \sum_{i\in  U}\Big( \Big(\frac{\subsetcountbatch}{\bsize}- \subsetprobbatch\Big)^2+\Big(\subsetprobbatch-  q  \Big)^2\Big) - 2 \sqrt{ \sum_{i\in  U}\Big(\frac{\subsetcountbatch}{\bsize}- \subsetprobbatch\Big)^2
\sum_{i\in  U}\Big(\subsetprobbatch-  q  \Big)^2}\\
& \ge |U| \Big( \frac{\subsetprobtarget(1-\subsetprobtarget)}{\bsize} - 24{\frac{ \epsilon\ln (e/\epsilon) } {\bsize}}-\frac{\eta}{2n} + \min_{i\in  U} (\subsetprobbatch-  q )^2\Big) \Big)  \\
&-2 |U| \sqrt{ \Big( \frac{\subsetprobtarget(1-\subsetprobtarget)}{\bsize} + 24{\frac{ \epsilon\ln (e/\epsilon)} {\bsize}}+\frac \eta {2n} \Big)
\max_{i\in  U}\Big(\subsetprobbatch-  q  \Big)^2}\\
&\ge |U| \Big( \frac{\subsetprobtarget(1-\subsetprobtarget)}{\bsize} - {\frac{24 \epsilon } {\bsize}}\ln \big(\frac e \epsilon\big)-\frac{\eta}{2n} +\min_{i\in  U} (\subsetprobbatch-  q )^2 -2 \sqrt{ \frac{16}{\bsize}}\,
\max_{i\in  U}\Big|\subsetprobbatch-  q  \Big|\Big)\\
&\ge |U| \Big( \frac{\subsetprobtarget(1-\subsetprobtarget)}{\bsize} - {\frac{24 \epsilon } {\bsize}}\ln \big(\frac e \epsilon\big)-\frac{\eta}{2n} +\big(|\subsetprobtarget -  q |-\frac \eta {2}\big)^2 -\frac{8}{\sqrt{ \bsize}}\,
\big(|\subsetprobtarget -  q |+\frac \eta {2}\big) \Big)
\end{align*}
Therefore,
\begin{align*}
&\sum_{i\in  U}\Big(\Big(\frac{\subsetcountbatch}{\bsize}-  q  \Big)^2 -   \frac{q(1-q)}{\bsize} \Big)\\
&\ge |U| \Big( -\frac{|\subsetprobtarget -  q |}{\bsize} - {\frac{24 \epsilon } {\bsize}}\ln \big(\frac e \epsilon\big)-\frac{\eta}{2n} +\big(|\subsetprobtarget -  q |-\frac \eta {2}\big)^2 -\frac{8}{\sqrt{ \bsize}}\,
\big(|\subsetprobtarget -  q |+\frac \eta {2}\big) \Big).
\end{align*}
This completes the proof of the lower bound. A similar calculation gives the desired upper bound as well.
\end{proof}
\end{comment}

